A Physics-Informed Meta-Learning Framework for the Continuous Solution of Parametric PDEs on Arbitrary Geometries

In this work, we introduce implicit Finite Operator Learning (iFOL) for the continuous and parametric solution of partial differential equations (PDEs) on arbitrary geometries. We propose a physics-informed encoder-decoder network to establish the mapping between continuous parameter and solution spaces. The decoder constructs the parametric solution field by leveraging an implicit neural field network conditioned on a latent or feature code. Instance-specific codes are derived through a PDE encoding process based on the second-order meta-learning technique. In training and inference, a physics-informed loss function is minimized during the PDE encoding and decoding. iFOL expresses the loss function in an energy or weighted residual form and evaluates it using discrete residuals derived from standard numerical PDE methods. This approach results in the backpropagation of discrete residuals during both training and inference. iFOL features several key properties: (1) its unique loss formulation eliminates the need for the conventional encode-process-decode pipeline previously used in operator learning with conditional neural fields for PDEs; (2) it not only provides accurate parametric and continuous fields but also delivers solution-to-parameter gradients without requiring additional loss terms or sensitivity analysis; (3) it can effectively capture sharp discontinuities in the solution; and (4) it removes constraints on the geometry and mesh, making it applicable to arbitrary geometries and spatial sampling (zero-shot super-resolution capability). We critically assess these features and analyze the network's ability to generalize to unseen samples across both stationary and transient PDEs. The overall performance of the proposed method is promising, demonstrating its applicability to a range of challenging problems in computational mechanics.

==> extra.tex <==
\iffalse
\textbf{Synthesizer Network} ($\mathcal{S}$)
At layer $l$, the synthesizer computes its output as follows:
\[
\mathbf{h}_s^{(l)} = \sigma\left( W_s^{(l)} \cdot \sin\left( \mathbf{x} \cdot \mathbf{b}_s^{(l)} \right) \right)
\]
where:
\begin{itemize}
  \item $\mathbf{h}_s^{(l)}$ is the output of the synthesizer at layer $l$,
  \item $W_s^{(l)}$ is the weight matrix at layer $l$,
  \item $\mathbf{b}_s^{(l)}$ is the frequency vector at layer $l$,
  \item $\sigma$ is the activation function (e.g., ReLU or tanh).
\end{itemize}

\textbf{Modulator Network} ($\mathcal{M}$)
Similarly, the modulator at layer $l$ is defined as:
\[
\mathbf{h}_m^{(l)} = \sigma\left( W_m^{(l)} \cdot \sin\left( \mathbf{x} \cdot \mathbf{b}_m^{(l)} \right) \right)
\]
where:
\begin{itemize}
  \item $\mathbf{h}_m^{(l)}$ is the output of the modulator at layer $l$,
  \item $W_m^{(l)}$ is the weight matrix at layer $l$,
  \item $\mathbf{b}_m^{(l)}$ is the frequency vector for the modulator at layer $l$.
\end{itemize}

At each layer, the synthesizer and modulator outputs are multiplied element-wise:
\[
\mathbf{h}^{(l)} = \mathbf{h}_s^{(l)} \odot \mathbf{h}_m^{(l)}
\]
where $\odot$ denotes element-wise multiplication.

\textbf{Meta-Learning}
The weights and frequency vectors are adapted via meta-learning. At each layer, the meta-parameters $\theta$ are updated based on the meta-objective $\mathcal{L}_\text{meta}$:
\[
\theta^{(l+1)} = \theta^{(l)} - \alpha \nabla_\theta \mathcal{L}_\text{meta}
\]
where $\alpha$ is the meta-learning rate and $\nabla_\theta \mathcal{L}_\text{meta}$ is the gradient of the meta-objective.

The final output of the network is computed by a readout layer:
\[
\hat{y} = W_o \cdot \mathbf{h}^{(L)} + b_o
\]
where:
\begin{itemize}
  \item $\mathbf{h}^{(L)}$ is the output from the last layer,
  \item $W_o$ is the output weight matrix,
  \item $b_o$ is the output bias term.
\end{itemize}


%\begin{figure}[H]
%  \centering
%\includegraphics[width=0.85\linewidth]{./Figs/NN_arch_1.jpg}
%  \caption{NN arch 1.}
%  \label{fig:NN_arch_1}
%\end{figure}

\fi




\color{black}
Applying the chain rule and variational calculus, the gradient of the loss function with respect to the predicted solution is given by:
\begin{equation}
\label{eq:cont_loss_variation}
\begin{aligned}
\delta_{u_{\theta, \gamma}}\mathcal{L}_{\mathbf{PDE}} & = \int_{\Omega}  \mathcal{R} \, d\Omega + \int_{\Omega} u_{\theta, \gamma} \,\delta_{u_{\theta, \gamma}}\mathcal{R} \, d\Omega  = \int_{\Omega}  \mathcal{R} \, d\Omega,
\end{aligned}
\end{equation}
where \(\delta_{u_{\theta, \gamma}}\mathcal{R}\) is zero due to the stationarity of the residual functional with respect to the solution field.


\begin{equation}
        M_{ij} = \int_{\Omega} \psi_i(x) \psi_j(x) \,d\Omega,
    \end{equation}



    

%Traditional numerical solvers are highly optimized for solving challenging PDE problems. However, they are typically designed for one-time use, requiring costly recomputation whenever input parameters change. Deep learning methods, particularly neural operators, offer a promising alternative but are often highly data-demanding. Integrating physical constraints into neural operators has shown potential in mitigating these challenges, yet training such complex networks remains difficult, especially across a wide range of input parameters. Furthermore, the application of neural operators to real-world problems is still underdeveloped, with key challenges including scalability to complex geometries, accuracy in capturing sharp gradients, and efficient training, all of which remain active areas of research.

%%Conditional neural fields represent a promising yet straightforward network architecture that compactly and continuously maps function spaces across arbitrary domains. They offer significant flexibility for operator learning in parametrized PDEs, as their outputs can be sampled at arbitrary resolutions and modified by adjusting a set of latent variables. In contrast to discrete networks, where memory usage increases inefficiently with spatio-temporal resolution, neural fields require memory that scales primarily with the number of parameters in the network. Additionally, specialized architectures, such as sinusoidal activations or Fourier features, enhance their ability to capture high-frequency details, while integration with numerical methods extends their applicability to complex geometries and topologies.
%This work aims to address some of the above challenges by integrating concepts from the standard finite element method and conditional neural fields into operator learning. As a result, we introduce a physics-informed encoder-decoder network to establish the mapping between continuous parameters and solution spaces for parametrized PDEs. To the best of our knowledge, this is the first application of a single-network conditional neural field for operator learning, owing to this capability to its unique loss formulation, which eliminates the need for the complex encode-process-decode pipeline \citep{serrano2023operator,catalani2024neural}. This approach is well-suited for complex geometries, offering data efficiency, requiring no labeled data, and demonstrating scalability to real-world industry applications, especially in the fields of materials engineering and science.


Operator learning faces several key challenges that hinder its broader adoption in scientific computing. 
\begin{itemize}
    \item A major issue is generalization, as models often struggle to extrapolate beyond training data, especially in highly nonlinear systems with complex geometries.   
    \item Capturing high-frequency features (discontinuous solution fields) remains challenging. In many industrial applications, one expects discontinuities in the solution fields which produce high gradients and therefore very relevant for design purposes (e.g. consider stress or flux values coming from derivation of the primary field such as displacement, or temperature). \color{black}
    \item Purely data-driven methodologies frequently demand substantial datasets generated through computationally intensive high-fidelity simulations or resource-demanding experimental campaigns. Moreover, existing operator-learning frameworks often do not explicitly encode physical constraints, thereby increasing the risk of generating solutions that are inconsistent with fundamental physical laws.
    \item The applicability to 3D problems with arbitrary geometries remains challenging due to both computational cost and accuracy limitations. In this context, the potential of meta-learning techniques is still underexplored, particularly in conditional learning of discontinuous fields on irregular meshes. \color{black}
\end{itemize}

==> iFOL/extra.tex <==
\iffalse
\textbf{Synthesizer Network} ($\mathcal{S}$)
At layer $l$, the synthesizer computes its output as follows:
\[
\mathbf{h}_s^{(l)} = \sigma\left( W_s^{(l)} \cdot \sin\left( \mathbf{x} \cdot \mathbf{b}_s^{(l)} \right) \right)
\]
where:
\begin{itemize}
  \item $\mathbf{h}_s^{(l)}$ is the output of the synthesizer at layer $l$,
  \item $W_s^{(l)}$ is the weight matrix at layer $l$,
  \item $\mathbf{b}_s^{(l)}$ is the frequency vector at layer $l$,
  \item $\sigma$ is the activation function (e.g., ReLU or tanh).
\end{itemize}

\textbf{Modulator Network} ($\mathcal{M}$)
Similarly, the modulator at layer $l$ is defined as:
\[
\mathbf{h}_m^{(l)} = \sigma\left( W_m^{(l)} \cdot \sin\left( \mathbf{x} \cdot \mathbf{b}_m^{(l)} \right) \right)
\]
where:
\begin{itemize}
  \item $\mathbf{h}_m^{(l)}$ is the output of the modulator at layer $l$,
  \item $W_m^{(l)}$ is the weight matrix at layer $l$,
  \item $\mathbf{b}_m^{(l)}$ is the frequency vector for the modulator at layer $l$.
\end{itemize}

At each layer, the synthesizer and modulator outputs are multiplied element-wise:
\[
\mathbf{h}^{(l)} = \mathbf{h}_s^{(l)} \odot \mathbf{h}_m^{(l)}
\]
where $\odot$ denotes element-wise multiplication.

\textbf{Meta-Learning}
The weights and frequency vectors are adapted via meta-learning. At each layer, the meta-parameters $\theta$ are updated based on the meta-objective $\mathcal{L}_\text{meta}$:
\[
\theta^{(l+1)} = \theta^{(l)} - \alpha \nabla_\theta \mathcal{L}_\text{meta}
\]
where $\alpha$ is the meta-learning rate and $\nabla_\theta \mathcal{L}_\text{meta}$ is the gradient of the meta-objective.

The final output of the network is computed by a readout layer:
\[
\hat{y} = W_o \cdot \mathbf{h}^{(L)} + b_o
\]
where:
\begin{itemize}
  \item $\mathbf{h}^{(L)}$ is the output from the last layer,
  \item $W_o$ is the output weight matrix,
  \item $b_o$ is the output bias term.
\end{itemize}


%\begin{figure}[H]
%  \centering
%\includegraphics[width=0.85\linewidth]{./Figs/NN_arch_1.jpg}
%  \caption{NN arch 1.}
%  \label{fig:NN_arch_1}
%\end{figure}

\fi




\color{black}
Applying the chain rule and variational calculus, the gradient of the loss function with respect to the predicted solution is given by:
\begin{equation}
\label{eq:cont_loss_variation}
\begin{aligned}
\delta_{u_{\theta, \gamma}}\mathcal{L}_{\mathbf{PDE}} & = \int_{\Omega}  \mathcal{R} \, d\Omega + \int_{\Omega} u_{\theta, \gamma} \,\delta_{u_{\theta, \gamma}}\mathcal{R} \, d\Omega  = \int_{\Omega}  \mathcal{R} \, d\Omega,
\end{aligned}
\end{equation}
where \(\delta_{u_{\theta, \gamma}}\mathcal{R}\) is zero due to the stationarity of the residual functional with respect to the solution field.


\begin{equation}
        M_{ij} = \int_{\Omega} \psi_i(x) \psi_j(x) \,d\Omega,
    \end{equation}



    

%Traditional numerical solvers are highly optimized for solving challenging PDE problems. However, they are typically designed for one-time use, requiring costly recomputation whenever input parameters change. Deep learning methods, particularly neural operators, offer a promising alternative but are often highly data-demanding. Integrating physical constraints into neural operators has shown potential in mitigating these challenges, yet training such complex networks remains difficult, especially across a wide range of input parameters. Furthermore, the application of neural operators to real-world problems is still underdeveloped, with key challenges including scalability to complex geometries, accuracy in capturing sharp gradients, and efficient training, all of which remain active areas of research.

%%Conditional neural fields represent a promising yet straightforward network architecture that compactly and continuously maps function spaces across arbitrary domains. They offer significant flexibility for operator learning in parametrized PDEs, as their outputs can be sampled at arbitrary resolutions and modified by adjusting a set of latent variables. In contrast to discrete networks, where memory usage increases inefficiently with spatio-temporal resolution, neural fields require memory that scales primarily with the number of parameters in the network. Additionally, specialized architectures, such as sinusoidal activations or Fourier features, enhance their ability to capture high-frequency details, while integration with numerical methods extends their applicability to complex geometries and topologies.
%This work aims to address some of the above challenges by integrating concepts from the standard finite element method and conditional neural fields into operator learning. As a result, we introduce a physics-informed encoder-decoder network to establish the mapping between continuous parameters and solution spaces for parametrized PDEs. To the best of our knowledge, this is the first application of a single-network conditional neural field for operator learning, owing to this capability to its unique loss formulation, which eliminates the need for the complex encode-process-decode pipeline \citep{serrano2023operator,catalani2024neural}. This approach is well-suited for complex geometries, offering data efficiency, requiring no labeled data, and demonstrating scalability to real-world industry applications, especially in the fields of materials engineering and science.


Operator learning faces several key challenges that hinder its broader adoption in scientific computing. 
\begin{itemize}
    \item A major issue is generalization, as models often struggle to extrapolate beyond training data, especially in highly nonlinear systems with complex geometries.   
    \item Capturing high-frequency features (discontinuous solution fields) remains challenging. In many industrial applications, one expects discontinuities in the solution fields which produce high gradients and therefore very relevant for design purposes (e.g. consider stress or flux values coming from derivation of the primary field such as displacement, or temperature). \color{black}
    \item Purely data-driven methodologies frequently demand substantial datasets generated through computationally intensive high-fidelity simulations or resource-demanding experimental campaigns. Moreover, existing operator-learning frameworks often do not explicitly encode physical constraints, thereby increasing the risk of generating solutions that are inconsistent with fundamental physical laws.
    \item The applicability to 3D problems with arbitrary geometries remains challenging due to both computational cost and accuracy limitations. In this context, the potential of meta-learning techniques is still underexplored, particularly in conditional learning of discontinuous fields on irregular meshes. \color{black}
\end{itemize}
